The Effects of Android Robots Displaying Emotion on Humans: Interactions between Older Adults and Android Robots

Often robots are seen as a means to an end to fulfill a logical objective task. Android robots, on the other hand, provide new possibilities to fulfill emotional tasks and could therefore be integrated into assistive scenarios. We explored this possibility by letting older adults and stakeholders have a conversation with an android robot capable of expressing emotion through facial expressions. The study was carried out with a wizard-of-oz approach and data collected with a mixed methods approach. We found that the participants were encouraged to speak more with the robot due to its smile. Simultaneously, many ethical questions were raised about transparency and manipulation. Our research can give valuable insight into the reaction of older adults to android robots that show emotions.

==> 6_Conclusion.tex <==
%\section{Conclusion}
% Future work
% our finding 




%This study is limited by the number of participants and the lengths of the interactions. In addition, the displayed emotions were not the central focus of the conversations. Instead, they were used spontaneously whenever they matched the context leading to a varying experience for each of the participants.
%Still, it could prove a fantastic potential for using the display of emotion to deepen the connection between humans and robots. Nevertheless, it cannot be disregarded that humanizing robots also carries a significant risk. When the distinctions between humans and robots become blurred, it may soon become impossible for some people to tell the two apart. Therefore, the risks and benefits need to be carefully evaluated, and it might also be reasonable to establish internationally binding guidelines to differentiate robots and humans visually.
%For now, it has to be clearly stated, though, that any of the participants experienced no difficulty in telling that they were not, in fact, interacting with a human, indicating that the robot is not that human-like after all 
%Many participants reported a positive reaction to being smiled at. However, the display of other, potentially more negative emotions, like sadness, fear, or anger, has to be evaluated in further study.
%Future research could solidify our result with quantitative data, directly comparing the interaction with robots who do and do not show emotions.
%It can also be concluded that context awareness and the feeling of being understood by the robot were reported as a more significant benefit than the idea of the robot feeling or communicating joy. It encouraged the participants to talk more, and it could be further investigated whether this effect could be achieved through other visual or auditory cues that are not directly related to a human-typical expression of happiness.
%The study could show that the display of emotion by an Android was generally seen as positive and beneficial but also shed light on the fact that there many ethical questions that need to be investigated. 
